FastTrack: Minimizing Stalls for CDN-based Over-the-top Video Streaming Systems

Traffic for internet video streaming has been rapidly increasing and is further expected to increase with the higher definition videos and IoT applications, such as 360 degree videos and augmented virtual reality applications. While efficient management of heterogeneous cloud resources to optimize the quality of experience is important, existing work in this problem space often left out important factors. In this paper, we present a model for describing a today's representative system architecture for video streaming applications, typically composed of a centralized origin server and several CDN sites. Our model comprehensively considers the following factors: limited caching spaces at the CDN sites, allocation of CDN for a video request, choice of different ports from the CDN, and the central storage and bandwidth allocation. With the model, we focus on minimizing a performance metric, stall duration tail probability (SDTP), and present a novel, yet efficient, algorithm to solve the formulated optimization problem. The theoretical bounds with respect to the SDTP metric are also analyzed and presented. Our extensive simulation results demonstrate that the proposed algorithms can significantly improve the SDTP metric, compared to the baseline strategies. Small-scale video streaming system implementation in a real cloud environment further validates our results.

==> abstract.tex <==
\begin{abstract}
Traffic for Over-the-top video streaming has been rapidly increasing. The traffic is further expected to increase with the higher definition videos and augmented reality applications. This necessitates efficient management of different cloud resources to optimize the quality of experience of the end users. This paper considers a CDN-based video streaming system where the cache at the CDN, allocation of CDN for a video request, choice of different ports from the CDN and the central storage, bandwidth allocation are all variables that can be decided. A novel two-stage probabilistic scheduling policy is proposed, and bounds for the stall duration tail probability are derived. A holistic optimization framework is developed to optimize a weighted user experience of all video files over the request scheduling probabilities, cache content placement, the bandwidth allocation among different streams,  and the modeling parameters in the bound. Efficient algorithm to solve the problem is proposed. The  experimental results demonstrate significant improvement in the QoE metric  as compared to the considered baseline strategies.
\end{abstract}







==> apdx_algs.tex <==
%\section{Algorithm Pseudo-codes for the Sub-problems}\label{apdx_table}


\begin{algorithm}[t]
\caption{NOVA Algorithm to solve Server Access and PSs selection Optimization sub-problem\label{alg:NOVA_Alg1Pi}}

\begin{enumerate}
\item \textbf{Initialize} $\nu=0$, $k=0$,$\gamma^{\nu}\in\left(0,1\right]$,
$\epsilon>0$,$\widetilde{\boldsymbol{\pi}}^{0}$ such that $\widetilde{\boldsymbol{\pi}}^{0}$
is feasible ,
\item \textbf{while} $\mbox{obj}\left(k\right)-\mbox{obj}\left(k-1\right)\geq\epsilon$
\item $\quad$//\textit{\small{}Solve for $\widetilde{\boldsymbol{\pi}}^{\nu+1}$ with
given $\widetilde{\boldsymbol{\pi}}^{\nu}$}{\small \par}
\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right),$
the solution of $\boldsymbol{\widehat{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)=$$\underset{\widetilde{\boldsymbol{\pi}}}{\text{argmin}}$
$\boldsymbol{\widetilde{U}}\left(\widetilde{\boldsymbol{\pi}},\widetilde{\boldsymbol{\pi}}^{\nu}\right)\,\, $ s.t.
$\left(\eqref{eq:rho_beta_d}--\eqref{eq:pi_q_p_gz}\right)$, $\left(\eqref{eq:mgf_beta_d}--
\eqref{eq:mgf_beta_e}\right)$, solved using  projected gradient descent 



\item $\quad$\textbf{Step 2}: $\ensuremath{\widetilde{\boldsymbol{\pi}}^{\nu+1}=\widetilde{\boldsymbol{\pi}}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)-\widetilde{\boldsymbol{\pi}}^{\nu}\right)}$.
\item $\quad$//\textit{\small{}update index}{\small \par}
\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
\item \textbf{end while}
\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)}$
\end{enumerate}
\end{algorithm}



\begin{algorithm}[ht]
	\caption{NOVA Algorithm to solve Auxiliary Variables  Optimization sub-problem\label{alg:NOVA_Alg1}}
	
	\begin{enumerate}
		\item \textbf{Initialize} $\nu=0$, $\gamma^{\nu}\in\left(0,1\right]$, $\epsilon>0$, $\boldsymbol{t}^{0}$ 
		such that $\boldsymbol{t}^{0}$  is feasible,
		\item \textbf{while} $\mbox{obj}\left(\nu\right)-\mbox{obj}\left(\nu-1\right)\geq\epsilon$
		\item $\quad$//\textit{\small{}Solve for  $\boldsymbol{t}^{\nu+1}$ with
			given $\boldsymbol{t}^{\nu}$}{\small \par}
		\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{t}}\left(\boldsymbol{t}^{\nu}\right),$
		the solution of  $\boldsymbol{\widehat{t}}\left(\boldsymbol{t}^{\nu}\right)=$$\underset{\boldsymbol{t}}{\text{argmin}}$
		$\boldsymbol{\overline{U}}\left(\boldsymbol{t},\boldsymbol{t}^{\nu}\right)$, s.t. \eqref{eq:t_leq_alpha_beta_d}--\eqref{eq:mgf_beta_e}, using projected gradient descent
\item $\quad$\textbf{Step 2}: $\ensuremath{\boldsymbol{t}^{\nu+1}=\boldsymbol{t}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{t}}\left(\boldsymbol{t}^{\nu}\right)-\boldsymbol{t}^{\nu}\right)}$.
		\item $\quad$//\textit{\small{}update index}{\small \par}
		\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
		\item \textbf{end while}
		\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{t}}\left(\boldsymbol{t}^{\nu}\right)}$
	\end{enumerate}
\end{algorithm}



\begin{algorithm}[ht]
	\caption{NOVA Algorithm to solve Bandwidth Allocation Optimization sub-problem\label{alg:NOVA_Alg3}}	
	\begin{enumerate}
		\item \textbf{Initialize} $\nu=0$, $\gamma^{\nu}\in\left(0,1\right]$, $\epsilon>0$, $\boldsymbol{w}^{0}$ 
		such that $\boldsymbol{w}^{0}$  is feasible,
		\item \textbf{while} $\mbox{obj}\left(\nu\right)-\mbox{obj}\left(\nu-1\right)\geq\epsilon$
		\item $\quad$//\textit{\small{}Solve for  $\boldsymbol{w}^{\nu+1}$ with
			given $\boldsymbol{w}^{\nu}$}{\small \par}
		\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{w}}\left(\boldsymbol{w}^{\nu}\right),$
		the solution of  $\boldsymbol{\widehat{w}}\left(\boldsymbol{w}^{\nu}\right)=$$\underset{\boldsymbol{b}}{\text{argmin}}$
		$\boldsymbol{\overline{U}}\left(\boldsymbol{w},\boldsymbol{w}^{\nu}\right)$, s.t. \eqref{eq:w_cde_gz}--
\eqref{eq:sum_w_de},\,\,\eqref{eq:t_leq_alpha_beta_d}--\eqref{eq:mgf_beta_e}, using projected gradient descent
		\item $\quad$\textbf{Step 2}: $\ensuremath{\boldsymbol{w}^{\nu+1}=\boldsymbol{w}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{w}}\left(\boldsymbol{w}^{\nu}\right)-\boldsymbol{w}^{\nu}\right)}$.
		\item $\quad$//\textit{\small{}update index}{\small \par}
		\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
		\item \textbf{end while}
		\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{w}}\left(\boldsymbol{w}^{\nu}\right)}$
	\end{enumerate}
\end{algorithm}






\begin{algorithm}[ht]
	\caption{NOVA Algorithm to solve Cache Placement Optimization sub-problem\label{alg:NOVA_Alg5}}
	
	\begin{enumerate}
		\item \textbf{Initialize} $\nu=0$, $\gamma^{\nu}\in\left(0,1\right]$, $\epsilon>0$, $\boldsymbol{L}^{0}$ 
		such that $\boldsymbol{L}^{0}$  is feasible,
		\item \textbf{while} $\mbox{obj}\left(\nu\right)-\mbox{obj}\left(\nu-1\right)\geq\epsilon$
		\item $\quad$//\textit{\small{}Solve for  $\boldsymbol{L}^{\nu+1}$ with
			given $\boldsymbol{L}^{\nu}$}{\small \par}
		\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{L}}\left(\boldsymbol{L}^{\nu}\right),$
		the solution of  $\boldsymbol{\widehat{L}}\left(\boldsymbol{L}^{\nu}\right)=$$\underset{\boldsymbol{L}}{\text{argmin}}$
		$\boldsymbol{\overline{U}}\left(\boldsymbol{L},\boldsymbol{L}^{\nu}\right)$, s.t. \eqref{eq:rho_beta_d}--
\eqref{eq:rho_nu_e},
\eqref{eq:capConst},
\eqref{eq:mgf_beta_d}-- \eqref{eq:mgf_beta_e}\\
		using projected gradient descent
		\item $\quad$\textbf{Step 2}: $\ensuremath{\boldsymbol{L}^{\nu+1}=\boldsymbol{L}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{L}}\left(\boldsymbol{L}^{\nu}\right)-\boldsymbol{L}^{\nu}\right)}$.
		\item $\quad$//\textit{\small{}update index}{\small \par}
		\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
		\item \textbf{end while}
		\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{L}}\left(\boldsymbol{L}^{\nu}\right)}$
	\end{enumerate}
\end{algorithm}


==> p_opt.tex <==
\subsubsection{PS Selection Probabilities}
Given the auxiliary variables, the bandwidth allocation weights, the streamed video quality probabilities, and the scheduling probabilities, this subproblem can be written as follows. 

\textbf{Input: $\boldsymbol{q}$, $\boldsymbol{b}$, $\boldsymbol{t}$, and $\boldsymbol{w}$}

\textbf{Objective:} $\qquad\quad\;\;$min $\left(\ref{eq:joint_otp_prob}\right)$

$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$s.t. 
\eqref{eq:rho_j},
\eqref{eq:Lambda_j},
\eqref{eq:sum_p_nuj},
\eqref{eq:don_pos_cond2},

$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$var. $\boldsymbol{p}$

 This optimization can be solved using NOVA algorithm. The constraints  \eqref{eq:rho_j}, \eqref{eq:Lambda_j}, \eqref{eq:sum_p_nuj}, and \eqref{eq:don_pos_cond2} are linear in $\boldsymbol{p}$, and hence, the domain is convex. 

 Algorithm \ref{alg:NOVA_Alg5} (given in Appendix \ref{apdx_table}) shows the used procedure to solve for $\boldsymbol{p}$. Let ${U_p}\left(\boldsymbol{p};\boldsymbol{p^\nu}\right)$ be the
convex approximation at iterate $\boldsymbol{p^\nu}$ to the original non-convex problem $U\left(\boldsymbol{p}\right)$, where $U\left(\boldsymbol{p}\right)$ is given by (\ref{eq:joint_otp_prob}), assuming other parameters constant. Then, a valid choice of  ${U_p}\left(\boldsymbol{p};\boldsymbol{p^\nu}\right)$ is the first order approximation of  $U\left(\boldsymbol{p}\right)$, i.e.,  
\begin{equation}
{U_p}\left(\boldsymbol{p},\boldsymbol{p^\nu}\right)=\nabla_{\boldsymbol{p}}U\left(\boldsymbol{p^\nu}\right)^{T}\left(\boldsymbol{p}-\boldsymbol{p^\nu}\right)+\frac{\tau_{p}}{2}\left\Vert \boldsymbol{p}-\boldsymbol{b^\nu}\right\Vert ^{2}.\label{eq:U_b}
\end{equation}
where $\tau_p$ is a regularization parameter. The detailed steps can be seen in Algorithm \ref{alg:NOVA_Alg5}. Since all the constraints  have been shown to be convex in $\boldsymbol{p}$, the optimization problem in Step 1 of  Algorithm \ref{alg:NOVA_Alg5} can be solved by the standard projected gradient descent algorithm. 

%Similar to Access  Optimization problem, we get the minimizer for (\ref{eq:U_t_u_bar}), step 1 in Algorithm \ref{alg:NOVA_Alg1}), and then continue until convergence. 


%In this sub-problem, we solve for all $t_i$, for fixed placement and given accessing probabilities. Similar to $\boldsymbol{\pi}$- Optimization problem, we used NOVA algorithm to solve for $t$.  Algorithm \ref{alg:NOVA_Alg1}, shows the used procedure to solve for $\boldsymbol{t}$. After initialization with feasible choice, NOVA keeps generating  a sequence of monotonically decreasing $\left\{ \boldsymbol{t}^{\nu+1}\right\} $ until  convergence.



\begin{lemma} \label{lem_t}

For fixed $\boldsymbol{t}$, $\boldsymbol{w}$, $\boldsymbol{b}$, and  $\boldsymbol{q}$, the optimization of our problem over 
$\boldsymbol{p}$ generates a sequence of monotonically decreasing
objective values and therefore is guaranteed to converge to a stationary point.
\end{lemma}
%\begin{proof}
%Since NOVA Algorithm generates a sequence of monotonically decreasing
%objective values as shown in \cite{scutNOVA}, $\boldsymbol{t}$ is guaranteed to converge to a stationary point.
%\end{proof}




==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
	\centering
	\includegraphics[trim=0in 0in 0in 0.0in, clip, width=.48\textwidth]{figs2/stallconvrg_final}
			\vspace{-.16in}
		\captionof{figure}{Convergence of mean stall duration.}
		\label{fig:ConvgMeanStall}
		\vspace{-.2in}
\end{figure}




\begin{figure*}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 4.1in 0in, clip, width=\textwidth]{figs2/stall_vs_ArrRate_final}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video arrival rates.}
		\label{fig:meanStallVsArrRate}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.1in 0in 4in 0in, clip, width=\textwidth]{figs2/qlty_vs_arrRate_final}
%		\vspace{-.3in}
		\captionof{figure}{Average quality for different video arrival rates.}
		\label{fig:meanQltyVsArrRate}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 4in 0in, clip,width=\textwidth]{figs2/stall_vs_VidSize_final}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video lengths.}
		\label{fig:meanStallVsVidSize} 
	\end{minipage}
%	\vspace{-.2in}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.1in 0in 4.8in 0in, clip, width=\textwidth]{figs2/qlty_vs_vidLen_final_v2}
%		\vspace{-.3in}
		\captionof{figure}{Average  quality for different video lengths.}
		\label{fig:meanQltyVsVidSize}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 3.8in 0in, clip, width=\textwidth]{figs2/qulty_stall_vs_VM_dj}
%		\vspace{-.3in}
		\captionof{figure}{Average video quality and mean stall duration for different number of parallel streams $d_j$.}
		\label{fig:qlty_stall_Vs_d_j}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.1in 0.1in 4.4in 0.1in, clip,width=\textwidth]{figs2/tradeOff_final_v2}
%		\vspace{-.3in}
		\captionof{figure}{Tradeoff between mean stall duration and  average streamed video quality obtained by varying $\theta$.}
		\vspace{-.15in}
		\label{fig:tradeoff} 
	\end{minipage}
%	\vspace{-.2in}


\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%













%\begin{figure}[t].
%		\centering
%	\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.35]{figs/stall_vs_ArrRate_all}
%			\vspace{-.2in}
%		\captionof{figure}{Mean stall duration for different video arrival rates. }
%		\label{fig:meanStallVsArrRate}
%		\vspace{-.18in}
%\end{figure}
%
%\begin{figure}[t]
%		\centering		\includegraphics[trim=0.1in 0in 0.0in 0.0in, clip,scale =0.35]{figs/qlty_vs_ArrRate_all}
%				\vspace{-.2in}
%		\captionof{figure}{Average quality for different video arrival rates.}
%		\label{fig:meanQltyVsArrRate}
%		\vspace{-.18in}
%\end{figure}


%\subsection{Mean Stall Duration optimization}
%In this subsection, we focus only on minimizing the mean stall duration of all files by setting $\theta=1$, {\em i.e.}, stall duration tail probability is not considered.% in this part of the simulation.

\subsubsection*{Convergence of the Proposed Algorithm}
Figure \ref{fig:ConvgMeanStall} shows the convergence  of our proposed algorithm, where we see the convergence of mean stall duration in about $2000$ iterations. 

% which alternatively optimizes the mean stall duration of all files over scheduling probabilities $\boldsymbol{\pi}$, auxiliary variables $\boldsymbol{t}$, quality probabilities $\boldsymbol{b}$, and bandwidth allocation weights $\boldsymbol{w}$. We notice that for $r=1000$ video files of size 600 sec with $m=12$ storage nodes and six quality levels shown in \ref{tab:DataRates}, the mean stall duration converges to the optimal value within less than $300$ iterations.  


\subsubsection*{Effect of Arrival Rate} We assume the arrival rate of all the files the same, and vary the arrival rates as depicted in Figures \ref{fig:meanStallVsArrRate} and \ref{fig:meanQltyVsArrRate}. These figures show the effect of different video arrival rates on the mean stall duration and  averaged quality, respectively. We note that PLQ-BTA achieves lowest stalls and lowest quality, since it fetches all videos at the lowest qualities. Similarly, PHQ-BTA has highest stalls, and highest video quality since it fetches all videos in the highest possible rate. The proposed algorithm has mean stall duration less than all the algorithms other than PLQ-BTA, and is very close to PLQ-BTA.  Further, the proposed algorithm has the highest video quality among all algorithms except PHQ-BTA and PEQ-BTA. Thus, the proposed algorithm helps optimize both the QoEs simultaneously achieving close to the best possible stall durations and achieving better average video quality than the baselines. With the choice of low $\theta$, the stall duration can be made very close to the stall duration achieved with the lowest quality while the proposed algorithm will still opportunistically increase quality of certain videos to obtain better average quality. 



%We compare our proposed algorithm with the six baseline  policies and see that the proposed algorithm outperforms all baseline strategies for the QoE metrics of mean stall duration and  average quality. Thus, sever access, VMs selection and bandwidth weights allocation of files are important for the reduction of mean stall duration. While the mean stall duration increases with arrival, our approach still maintain low mean stall duration compared to the baselines. Moreover, we observe that the algorithms that optimize the quality tend to increase the quality of the streamed video only if the stall durations are zero (or close to zero) and adopt the lowest quality if the stall durations are not zero.
%Figure \ref{fig:meanQltyVsArrRate}
%shows that PLQ-BTA (PHQ-BTA) streaming policy realizes the lowest (highest) mean stall duration as it is aggressively minimize (maximize) the stall (quality) at the cost of other optimized parameters.


%Intuitively, having optimized placement leads to less stall duration (for all policies) since video chunks are balanced across the different storage nodes. Hence, the possibility of congested bottleneck nodes reduces accordingly. While mean stall duration increases as arrival rate increases, our approach, unlike PEAP and BNW, does not explode  as others do (especially for optimized one). 

\subsubsection*{Effect of Video Length}
The effect of having different video lengths on the mean stall duration and  average quality is also captured in Figures \ref{fig:meanStallVsVidSize} and \ref{fig:meanQltyVsVidSize}, respectively, where we assume that all the videos are of the same length. Apparently, the mean stall duration increases with the video length while the average quality decreases with the video length. The qualitative comparison of the different algorithms is the same as described in the case of varying arrival rates. Thus, at $\theta = 10^{-7}$, the proposed algorithm achieves the mean stall duration close to that of  PLQ-BTA while achieving significantly better quality. For algorithms other than PLQ-BTA, PEQ-BTA, and PHQ-BTA, the proposed algorithms outperforms all other baselines in both the metrics. %We also note that a fixed $\theta$ is used, and thus the average quality term gets more preference as the video lengths increase. Thus, for higher video lengths, 



%larger video sizes may incur more stalls as compared to the small ones since the chance of getting delayed chunks is increased. However, our proposed approach gives the lowest mean stall duration compared to the considered baselines. Since we magnify stall minimization over quality enhancement, the controlled-quality based algorithms stream the video with base-layer (the lowest possible) quality when the stalls are not equal to zero and stream with higher quality only if the stalls are zero. The greedy-based approaches (PLQ-BTA and PHQ-BTA) look into one metric to signify without taking the another one into account which results in performing the worst among all other algorithms with respect to the non-optimized parameter. For example, PHQ-BTA achieves the highest quality but, on the hand, realizes the highest mean stall duration. Finally, we note that the proposed optimization strategy effectively reduces the mean stall duration (while maintaining smooth streamed video) and outperforms the considered baseline strategies. Thus, joint optimization over all optimized parameters helps reduce the mean stall duration significantly and optimize the  average quality.


%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_7_mean_stall_NoOfFiles_source.eps}
%\caption{Mean stall duration for different number of video files with different video sizes. \label{fig:meanStallNumFiles} }
%\end{figure}


%\subsubsection*{Effect of the Number of Video Files}
%
%Figure \ref{fig:meanStallNumFiles} demonstrates the impact of varying the number of video files from $200$ files to $1000$ files  on the mean stall duration, where the video lengths are generated according to Pareto distribution with the same parameter defined earlier (scale of 300, and shape of 2).  We note that the proposed optimization strategy effectively reduces the mean stall duration and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{t}$,  $\boldsymbol{\pi}$,  $\boldsymbol{w}$, and  $\boldsymbol{b}$ helps reduce the mean stall duration significantly.


%\subsection{Average Quality  Optimization}
%
%In this subsection, we consider optimizing (magnifying) the quality of the streamed video by maximizing the quality probabilities, $\boldsymbol{b}$, by setting $0.5\leq\theta_{q}\leq1$
% in (\ref{eq:joint_otp_prob}).
%
%\subsubsection*{Varying Quality factor parameter}
%Figure \ref{fig:meanStallVsArrRate} 
% shows the average quality of the streamed videos versus the
%stall factor $\theta_{s}$ for the selected set of algorithms. Apparently,
%our proposed approach gives the highest quality as it aggressively
%maximizes the quality over the stall duration, i.e., streaming the
%larger videos by the highest possible probability. These results show
%also the greedy behavior of our proposed approach as $\theta_{q}$  increases (or alternatively $\theta_{s}$ decreases) and clearly at $\theta_{q}=1$ (that is, $\theta_{s}=0$) our approach streams the video of the largest size and thus the average quality of the streamed video is
%$\ell=6$, i.e., which is the highest possible quality. 


%\begin{figure}[t]
%		\centering
%		\includegraphics[trim=0.1in 0in 0.0in 0.1in, clip, scale =0.30]{figs/stall_vs_vidSize_all}
%		\vspace{-.2in}
%		\captionof{figure}{Mean stall duration for different video lengths.}
%		\label{fig:meanStallVsVidSize} 
%		\vspace{-.18in}
%	\end{figure}%












%\begin{figure*}
%	\centering
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.1in 0in 5in 0in, clip, width=\textwidth]{figs/qlty_vs_vidSize_all}
%%		\vspace{-.3in}
%		\captionof{figure}{Average streamed quality for different video lengths.}
%		\label{fig:meanQltyVsVidSize}
%	\end{minipage}%
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.1in 0in 5in 0in, clip, width=\textwidth]{figs/qlty_stall_vs_d_j2}
%%		\vspace{-.3in}
%		\captionof{figure}{Average video quality and mean stall duration for different number of parallel streams $d_j$.}
%		\label{fig:qlty_stall_Vs_d_j}
%	\end{minipage}
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0in 0in 5in 0in, clip,width=\textwidth]{figs/tradeOff}
%%		\vspace{-.3in}
%		\captionof{figure}{Tradeoff between mean stall duration and  average streamed video quality obtained by varying $\theta$.}
%		\label{fig:tradeoff} 
%	\end{minipage}
%%	\vspace{-.2in}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


















%\begin{figure}[t]
%		\centering
%		\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.30]{figs/qlty_vs_vidSize_all}
%		\vspace{-.2in}
%		\captionof{figure}{ Average streamed quality for different video lengths.}
%		\label{fig:meanQltyVsVidSize}
%		\vspace{-.18in}
%	\end{figure}
%
%
%	\begin{figure}[t]
%		\centering
%	\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.35]{figs/qlty_stall_vs_d_j2}
%		\vspace{-.2in}
%		\captionof{figure}{Average video quality and mean stall duration for different number of parallel streams $d_j$.}
%		\label{fig:qlty_stall_Vs_d_j}
%		\vspace{-.18in}
%	\end{figure}





%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_8_stallTail_vs_Num_iterations_source2.eps}
%\caption{Stall duration Tail Probability for different $x$. \label{fig:congStallDiffXvalues} }
%\end{figure}

%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_9_wieghtedLat_vs_x_comp_logy_source.eps}
%\caption{Stall duration tail probability for different $x$ (in seconds). \label{fig:tailProbDiffX} }
%\end{figure}
\subsubsection*{ Effect of the Number of the Parallel Streams ($d_j$)}
Figure \ref{fig:qlty_stall_Vs_d_j} plots the average   streamed video quality and mean stall duration for varying number of parallel streams, $d_j$, for our proposed algorithm. We vary the number of PSs from $10$ to $70$ with increment step of 10 with $\theta=10^{-7}$. Increasing $d_j$ can only improve performance since some of the bandwidth splits can be zero thus giving the lower $d_j$ solution as one of the possible feasible solution. Increasing $d_j$ thus decreases stall durations by having more parallel streams, while increasing average quality. We note that for $d_j<50$, mean stall duration is non-zero and the stall duration decreases significantly while the average quality increases only slightly.  For $d_j>50$, the stall duration remains zero and the average video quality increases significantly with increase in $d_j$. Even though larger $d_j$ gives better results, the server may only be able to handle a limited parallel connections thus limiting the value of $d_j$ in the real systems. 



 %Intuitively, we can see that the stall duration decreases as the number of VMs ($d_j$) increases since more jobs (videos) can be handled (streamed) simultaneously.
 
%  Further, when the mean stall duration is not zero, the proposed algorithm streams the video with approximately base-layer quality as we prioritize the stall minimization over the quality improvement by setting $\theta_q=10^{-7}$. Thus, more videos are concurrently streamed with close to base-layer quality. On contrary, when the mean stall duration is zero, the algorithm starts improving the quality. Hence, the proposed algorithm manages to significantly improve the two QoE metrics as $d_j$ increases. 
%\begin{figure*}
%	\centering
%%	\begin{minipage}{.32\textwidth}
%%		\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/tradeOff}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for different arrival rates for video files ($x=150$ s).}
%%		\label{fig:tailProbArrRate}
%%	\end{minipage}%
%%		\hspace{2mm}
%%		\begin{minipage}{.32\textwidth}
%%			\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/convgstall2}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for varying number of video files ($x=150$ s).}
%%		\label{fig:Fig_9_stallLat_vs_NumOfFiles}
%%		\end{minipage}
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and stall duration tail probability obtained by varying $\theta$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure*}

%\begin{figure}[t]
%	\centering
%			\centering
%	\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.35]{figs/tradeOff}
%			\vspace{-.2in}
%			\captionof{figure}{Tradeoff between mean stall duration and  average streamed video quality obtained by varying $\theta$.}
%			\label{fig:tradeoff}
%			\vspace{-.18in}
%\end{figure}

\vspace{-.05in}
\subsubsection*{Tradeoff  between mean stall duration and  average video quality}


The preceding results show a trade off between the mean stall duration and
the  average quality of the streamed video. In order to investigate such tradeoff, Figure \ref{fig:tradeoff} plots the  average video quality versus the mean stall duration for different values of $\theta$ ranging from $\theta=10^{-8}$ to $\theta=10^{-4}$. This figure implies that a compromise between the two QoE metrics can be achieved by our proposed streaming algorithm by setting $\theta$  to an appropriate value. As expected, increasing $\theta$ will increase the mean stall duration as there is more priority to maximizing the average video quality.   Thus, an efficient tradeoff point between the QoE metrics can be chosen based on the service quality level desired by the service provider. %based on the point on the curve that is appropriate for the clients.

==> sec_5_NumericalResults2.tex <==
\section{Numerical Results}\label{sec:num}
In this section, we evaluate our proposed  algorithm for optimization of mean and tail probability of stall duration and show the effect of the trade-off of parameter $\theta$. We first study the two extremes where only either mean stall duration objective or tail stall duration probability is considered. Then, we show the tradeoff between the two QoE metrics based on the trade-off parameter $\theta$.

%how the impact of the tradeoff objective function varies with respect to the trade-off factor.  



\begin{table}[b]
{\caption{Storage Node Parameters Used in our Simulation (Shift $\beta=10msec$
and rate $\alpha$ in 1/s)}
}


\resizebox{.49\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Node 1}} & \multicolumn{1}{c}{\textbf{Node 2}} & \multicolumn{1}{c}{\textbf{Node 3}} & \multicolumn{1}{c}{\textbf{Node 4}} & \multicolumn{1}{c}{\textbf{Node 5}} & \multicolumn{1}{c}{\textbf{Node 6}}\tabularnewline
\hline 
{$\alpha_{j}$} & {$18.2298$} & {$24.0552$} & {$11.8750$} & {$17.0526$} & {$26.1912$} & {$23.9059$}\tabularnewline
\hline 
\end{tabular}}

\resizebox{.5\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Node 7}} & \multicolumn{1}{c}{\textbf{Node 8}} & \multicolumn{1}{c}{\textbf{Node 9}} & \multicolumn{1}{c}{\textbf{Node 10}} & \multicolumn{1}{c}{\textbf{Node 11}} & \multicolumn{1}{c}{\textbf{Node 12}}\tabularnewline
\hline 
{$\alpha_{j}$} & {$27.006$} & {$21.3812$} & {$9.9106$} & {$24.9589$} & {$26.5288$} & {$21.8067$}\tabularnewline
\hline 
\end{tabular}\label{tab:Storage-Nodes-Parameters}
}
\end{table}

\subsection{Numerical Setup}
 We simulate our algorithm in a distributed storage system of $m=12$ distributed nodes, where each video file uses an $(7,4)$ erasure code. We consider $r=1000$ files, whose sizes are generated based on Pareto distribution \cite{arnold2015pareto} with shape factor of $2$ and scale of $300$, respectively. Thus, the first $1000$ file-sizes that are less than 40 minutes are chosen.  We also assume that the chunk service time  follows a shifted-exponential distribution with rate $\alpha_{j}$ and shift $\beta_{j}$, whose values are shown in Table 2, which are generated at random and kept fixed for the experiments. Unless explicitly stated, the arrival rate for the first $500$ files is $0.002s^{-1}$ while for the next $500$ files is set to be $0.003s^{-1}$. Chunk size $\tau$ is set to be equal to $4$ s. When generating video files, the sizes of the video file sizes are rounded up to the multiple of $4$ sec. We note that a high load scenario is considered for the numerical results. In practice, the load will not be that high. However, higher load helps demonstrate the significant improvement in performance as compared to the lightly loaded scenarios where there are almost no stalls. In order to initialize our algorithm, we use a random placement of files on all the servers. Further, we set $\pi_{ij}=k/n$ on the placed servers with $t_{i}=0.01$ $\forall i$ and $j \in \mathcal{S}_{i}$. However, these choices of $\pi_{ij}$ and $t_{i}$ may not be feasible. Thus, we modify the initialization of  $\boldsymbol{\pi}$  to be closest norm feasible solution  given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$.  We  compare our proposed approach with three strategies:
 \begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
\item {\em Random Placement, Optimized Access (RP-OA): }  In this strategy, the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Given the random placement, the variables $\boldsymbol{t}$ and $\boldsymbol{\pi}$ are optimized using the Algorithm in Section \ref{sec:algo}, where $\boldsymbol{\mathcal{S}}$-optimization is not performed.

\item {\em Optimized Placement, Projected Equal Access (OP-PEA): }
The strategy utilizes $\boldsymbol{\pi}$, $\boldsymbol{t}$ and $\boldsymbol{\mathcal{S}}$ as mentioned in the setup. Then, alternating optimization over placement and $\boldsymbol{t}$ are performed using the proposed algorithm.

 %In this strategy, the placement is optimized while the access is chosen equally likely at the servers chosen. In order to do that, we perform an iterative algorithm as in Section \ref{sec:algo}, where the $\boldsymbol{\pi}$-optimization is replaced by taking $\pi_{ij}=k/n$ $\forall i$ and $j \in \mathcal{S}_{i}$ and projecting $\boldsymbol{\pi}$ to the feasible set by finding the closest norm feasible solution given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$.


\item {\em Random Placement, Projected Equal Access (RP-PEA): } In this strategy, the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Further, we set $\pi_{ij}=k/n$ on the placed servers with $t_{i}=0.01$ $\forall i$ and $j \in \mathcal{S}_{i}$. We then modify the initialization of $\boldsymbol{\pi}$ to be closest norm feasible solution  given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$. Finally, an optimization over $\boldsymbol{t}$ is performed to the objective using Algorithm (\ref{alg:NOVA_Alg1}).


\end{enumerate} 
 
\begin{figure*}[htb]
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 0in 0.0in, clip, width=\textwidth]{figs/convgstall2}
		%	\vspace{-.3in}
		\captionof{figure}{Convergence of mean stall duration.}
		\label{fig:ConvgMeanStall}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_vs_rate2}
		%	\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video arrival rates with different video lengths. }
		\label{fig:meanArrRateSameSize}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip,width=\textwidth]{figs/stall_vidSize}
		%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video sizes considering  $\ell=3$.  }
		\label{fig:meanArrRateDiffSize}
	\end{minipage}
	%\vspace{-.2in}
	
	\vspace{-.1in}
\end{figure*}


\subsection{Mean Stall Duration optimization}
In this subsection, we focus only on minimizing the mean stall duration of all files by setting $\theta=1$, {\em i.e.}, stall duration tail probability is not considered.% in this part of the simulation.

\subsubsection*{Convergence of the Proposed Algorithm}
Figure \ref{fig:ConvgMeanStall} shows the convergence  of our proposed algorithm, which alternatively optimizes the mean stall duration of all files over scheduling probabilities $\boldsymbol{\pi}$, auxiliary variables $\boldsymbol{t}$, quality probabilities $\boldsymbol{b}$, and bandwidth allocation weights $\boldsymbol{w}$. We notice that for $r=1000$ video files of size 600 sec with $m=12$ storage nodes and six quality levels shown in \ref{tab:DataRates}, the mean stall duration converges to the optimal value within less than $300$ iterations.  


\subsubsection*{Effect of Arrival Rate} Figures \ref{fig:meanArrRateSameSize}  shows the effect of different video arrival rates on the mean stall duration for different-size video  whose lengths follow the Pareto-distributed described above.  We compare our proposed algorithm with the three baseline  policies and see that the proposed algorithm outperforms all baseline strategies for the QoE metric of mean stall duration. Thus, both access and bandwidth weights allocation of files are both important for the reduction of mean stall duration. We see that the mean stall duration increases with arrival rates. However, our approach still maintain low mean stall duration compared to the baselines.


%Intuitively, having optimized placement leads to less stall duration (for all policies) since video chunks are balanced across the different storage nodes. Hence, the possibility of congested bottleneck nodes reduces accordingly. While mean stall duration increases as arrival rate increases, our approach, unlike PEAP and BNW, does not explode  as others do (especially for optimized one). 

\subsubsection*{Effect of Video Size}
The effect of having different video sizes is also captured in Figure (\ref{fig:meanArrRateDiffSize}). Clearly, larger video sizes may incur more stalls compared to small ones as the chance of getting delayed chunks is increased. However, our proposed approach gives the lowest mean stall duration compared to the considered baselines.
%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_7_mean_stall_NoOfFiles_source.eps}
%\caption{Mean stall duration for different number of video files with different video sizes. \label{fig:meanStallNumFiles} }
%\end{figure}


\subsubsection*{Effect of the Number of Video Files}

Figure \ref{fig:meanStallNumFiles} demonstrates the impact of varying the number of video files from $200$ files to $1000$ files  on the mean stall duration, where the video lengths are generated according to Pareto distribution with the same parameter defined earlier (scale of 300, and shape of 2).  We note that the proposed optimization strategy effectively reduces the mean stall duration and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{t}$,  $\boldsymbol{\pi}$,  $\boldsymbol{w}$, and  $\boldsymbol{b}$ helps reduce the mean stall duration significantly.


\subsection{Average Quality  Optimization}

In this subsection, we consider optimizing (magnifying) the quality of the streamed video by maximizing the quality probabilities, $\boldsymbol{b}$, by setting $0.5\leq\theta_{q}\leq1$
 in (\ref{eq:joint_otp_prob}).

\subsubsection*{Varying Quality factor parameter}
Figure \ref{fig:congStallDiffXvalues} 
 shows the average quality of the streamed videos versus the
stall factor $\theta_{s}$ for the selected set of algorithms. Apparently,
our proposed approach gives the highest quality as it aggressively
maximizes the quality over the stall duration, i.e., streaming the
larger videos by the highest possible probability. These results show
also the greedy behavior of our proposed approach as $\theta_{q}$  increases (or alternatively $\theta_{s}$ decreases) and clearly at $\theta_{q}=1$ (that is, $\theta_{s}=0$) our approach streams the video of the largest size and thus the average quality of the streamed video is
$\ell=6$, i.e., which is the highest possible quality. 


\begin{figure*}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_NoOfVid}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different number of video files with different video lengths.}
		\label{fig:meanStallNumFiles} 
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/qualty_vs_theta_q}
%		\vspace{-.3in}
		\captionof{figure}{ Average Streamed Quality versus quality factor $\theta_q$}
		\label{fig:congStallDiffXvalues}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 0.1in 0in, clip,width=\textwidth]{figs/qlty_stall_vs_d}
%		\vspace{-.3in}
		\captionof{figure}{Average Video Quality and Mean Stall duration versus the number of virtual queues $d$}
		\label{fig:tailProbDiffX}
	\end{minipage}
%	\vspace{-.2in}

\vspace{-.15in}
\end{figure*}




%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_8_stallTail_vs_Num_iterations_source2.eps}
%\caption{Stall duration Tail Probability for different $x$. \label{fig:congStallDiffXvalues} }
%\end{figure}

%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_9_wieghtedLat_vs_x_comp_logy_source.eps}
%\caption{Stall duration tail probability for different $x$ (in seconds). \label{fig:tailProbDiffX} }
%\end{figure}
\subsubsection*{ Effect of the Number of the Virtual Queues $d$}
Figure \ref{fig:tailProbDiffX} plots the 
average of the streamed video quality and mean stall duration versus the number of virtual queses $d$. We vary the number of VQs from 5 to 30 with increment step of 5 and we set $\theta_q=1e-6$. We can see that the stall duration decreases as the number of VQs increases since more jobs can be handled simultaneously. We also observe that the proposed algorithm gives higher quality as $d$ increases which results from serving more than a job concurrently and allows for larger videos to be served. Hence, the proposed algorithm manages to significantly improve the two QoE metrics as $d$ increases.

%\begin{figure*}
%	\centering
%%	\begin{minipage}{.32\textwidth}
%%		\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/tradeOff}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for different arrival rates for video files ($x=150$ s).}
%%		\label{fig:tailProbArrRate}
%%	\end{minipage}%
%%		\hspace{2mm}
%%		\begin{minipage}{.32\textwidth}
%%			\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/convgstall2}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for varying number of video files ($x=150$ s).}
%%		\label{fig:Fig_9_stallLat_vs_NumOfFiles}
%%		\end{minipage}
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and stall duration tail probability obtained by varying $\theta$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure*}

\begin{figure}[t]
	\centering
%		\hspace{2mm}
		\begin{minipage}{.32\textwidth}
			\centering
			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
	%		\vspace{-.3in}
			\captionof{figure}{Tradeoff between mean stall duration and streamed video quality obtained by varying $\theta_s$.  }
			\label{fig:tradeoff}
		\end{minipage}
	
		\vspace{-.2in}
\end{figure}


\subsection{Tradeoff  between mean stall duration and video quality}


The preceding results show a trade off between the mean stall duration and
the streamed quality. In order to investigate such tradeoff, Figure \ref{fig:tradeoff} plots the average video quality versus the mean stall duration for different values of $\theta$ ranging from $\theta=10^{-5}$ to $\theta=10^{-7}$. This figure implies that a compromise between the two QoE metrics can be achieved by our proposed   streaming algorithm by setting the quality and stall factors ($\theta_q$ and $\theta_s$) to proper values. As expected, increasing $\theta_s$ will reduce the mean stall duration as higher priority is giving to minimize the stall over the quality. Thus, an efficient tradeoff point between the QoE metrics can be chosen based on the point on the curve that is appropriate for the clients.


